Correlations between $\ensuremath{\mit{\Upsilon}(n\text{S})}\xspace$ production and the underlying event in $\ensuremath{p\!p}\xspace$ collisions with the ATLAS detector

Recent studies from various experiments at the LHC and RHIC suggest that small collision systems exhibit quark-gluon plasma (QGP) like signatures that were typically observed in large systems. While QGP like signatures have been observed in the soft sector, strong constraints on possible partonic energy loss were established in the hard sector. At the same time, there are multiple pieces of evidence pointing to correlations between hard and soft particle production in proton-proton collisions. The correlations between hard and soft particle production in $pp$ collisions are studied in events with $\Upsilon$ mesons, which provide a valuable hard probe to study such effects. The multiplicity and distributions of kinematic variables of charged particles produced in association with an $\Upsilon$ meson are measured using 139 fb$^{-1}$ of data at $\ensuremath{\sqrt{s}}\xspace = 13$~TeV collected by the ATLAS experiment at the LHC. The measurement is performed separately for the first three $\Upsilon$(nS) states in intervals of their transverse momentum. At low transverse momentum, the associated charged-particle multiplicity is observed to be systematically lower in collisions where $\Upsilon$(2S) or $\Upsilon$(3S) is produced compared to $\Upsilon$(1S), with the difference decreasing as the $\Upsilon$ transverse momentum increases.

==> defs.tex <==
% defs.tex -- macro definitions for the DIS2026 PoS proceedings

\RequirePackage{xspace}
\RequirePackage{ifthen}
% amsmath, graphicx and xcolor are already loaded by pos.sty.

%-------------------------------------------------------------------------------
% Units
%-------------------------------------------------------------------------------

% Departure 1: plain switch in place of the kvoptions eVkern option.
\newif\ifeVkern
\eVkernfalse

\ifeVkern
  \newcommand*{\electronvolt}{\text{e\kern-0.1em V}}
\else
  \newcommand*{\electronvolt}{eV}
\fi

\newcommand*{\TeV}{\ensuremath{\text{T\electronvolt}}\xspace}
\newcommand*{\GeV}{\ensuremath{\text{G\electronvolt}}\xspace}
\newcommand*{\MeV}{\ensuremath{\text{M\electronvolt}}\xspace}
\newcommand*{\keV}{\ensuremath{\text{k\electronvolt}}\xspace}
\newcommand*{\eV}{\ensuremath{\text{\electronvolt}}\xspace}

\newcommand*{\TeVc}{\ensuremath{\text{T\electronvolt/}c}\xspace}
\newcommand*{\GeVc}{\ensuremath{\text{G\electronvolt/}c}\xspace}
\newcommand*{\MeVc}{\ensuremath{\text{M\electronvolt/}c}\xspace}
\newcommand*{\keVc}{\ensuremath{\text{k\electronvolt/}c}\xspace}
\newcommand*{\eVc}{\ensuremath{\text{\electronvolt/}c}\xspace}

\newcommand*{\TeVcc}{\ensuremath{\text{T\electronvolt/}c^{2}}\xspace}
\newcommand*{\GeVcc}{\ensuremath{\text{G\electronvolt/}c^{2}}\xspace}
\newcommand*{\MeVcc}{\ensuremath{\text{M\electronvolt/}c^{2}}\xspace}
\newcommand*{\keVcc}{\ensuremath{\text{k\electronvolt/}c^{2}}\xspace}
\newcommand*{\eVcc}{\ensuremath{\text{\electronvolt/}c^{2}}\xspace}

\newcommand*{\ifb}{\mbox{fb\(^{-1}\)}\xspace}
\newcommand*{\ipb}{\mbox{pb\(^{-1}\)}\xspace}
\newcommand*{\inb}{\mbox{nb\(^{-1}\)}\xspace}

\newcommand*{\degr}{\ensuremath{^\circ}}

\let\tev=\TeV
\let\gev=\GeV
\let\mev=\MeV
\let\kev=\keV
\let\ev=\eV

\let\tevc=\TeVc
\let\gevc=\GeVc
\let\mevc=\MeVc
\let\kevc=\keVc
\let\evc=\eVc

\let\tevcc=\TeVcc
\let\gevcc=\GeVcc
\let\mevcc=\MeVcc
\let\kevcc=\keVcc
\let\evcc=\eVcc

\newcommand*{\tesla}{\ensuremath{\text{T}}\xspace}
\newcommand*{\metre}{\ensuremath{\text{m}}\xspace}

%-------------------------------------------------------------------------------
% Generators and simulation
%-------------------------------------------------------------------------------

\newcommand*{\Pythia}{\textsc{Pythia}\,8\xspace}
\newcommand*{\Herwig}{\textsc{Herwig}\xspace}
\newcommand*{\Sherpa}{\textsc{Sherpa}\xspace}
\newcommand*{\Angantyr}{\textsc{Angantyr}\xspace}
\newcommand*{\Geant}{\textsc{Geant4}\xspace}
\newcommand*{\Photos}{\textsc{Photos}\xspace}

%-------------------------------------------------------------------------------
% Collision systems and centre-of-mass energy
%-------------------------------------------------------------------------------

\newcommand*{\pps}{\ensuremath{p\!p}\xspace}
\newcommand*{\ppb}{\ensuremath{p\mathrm{Pb}}\xspace}
\newcommand*{\pPb}{\ensuremath{p+\mathrm{Pb}}\xspace}
\newcommand*{\PbPb}{\ensuremath{\mathrm{Pb}+\mathrm{Pb}}\xspace}

\newcommand*{\s}{\ensuremath{\sqrt{s}}\xspace}
\newcommand*{\sn}{\ensuremath{\sqrt{s_{_{\mathrm{NN}}}}}\xspace}

%-------------------------------------------------------------------------------
% Quarkonium states
%-------------------------------------------------------------------------------

\newcommand*{\Upsa}{\ensuremath{\mit{\Upsilon}}\xspace}
\newcommand*{\Upsn}{\ensuremath{\mit{\Upsilon}(n\text{S})}\xspace}
\newcommand*{\UpsOne}{\ensuremath{\mit{\Upsilon}(\text{1S})}\xspace}
\newcommand*{\UpsTwo}{\ensuremath{\mit{\Upsilon}(\text{2S})}\xspace}
\newcommand*{\UpsThree}{\ensuremath{\mit{\Upsilon}(\text{3S})}\xspace}
\newcommand*{\UpsMs}{\ensuremath{\mit{\Upsilon}(m\text{S})}\xspace}
\let\Uone=\UpsOne
\let\Utwo=\UpsTwo
\let\Uthree=\UpsThree

\newcommand*{\chib}{\ensuremath{\chi_{b}(m\text{P})}\xspace}

% Departure 2: lower-case psi, as in the PDG.
\newcommand*{\jpsi}{\ensuremath{J/\psi}\xspace}
\newcommand*{\psits}{\ensuremath{\psi(\text{2S})}\xspace}
%\newcommand*{\jpsi}{\ensuremath{J/\mit{\Psi}}\xspace}
%\newcommand*{\psits}{\ensuremath{\mit{\Psi}(\text{2S})}\xspace}

%-------------------------------------------------------------------------------
% Quark pairs
%-------------------------------------------------------------------------------

\newcommand*{\uds}{\textit{u,d,s}\xspace}
\newcommand*{\qqbar}{\ensuremath{q\bar{q}}\xspace}
\newcommand*{\chum}{\ensuremath{c\bar{c}}\xspace}
\newcommand*{\btum}{\ensuremath{b\bar{b}}\xspace}

\newcommand*{\equm}{\ensuremath{(q\bar{q})^{\star}}\xspace}
\newcommand*{\echum}{\ensuremath{(c\bar{c})^{\star}}\xspace}
\newcommand*{\ebtum}{\ensuremath{(b\bar{b})^{\star}}\xspace}

\newcommand*{\ohf}{\ensuremath{q||\bar{q}}\xspace}
\newcommand*{\ochm}{\ensuremath{c||\bar{c}}\xspace}
\newcommand*{\obtm}{\ensuremath{b||\bar{b}}\xspace}

%-------------------------------------------------------------------------------
% Charged-particle and event observables
%-------------------------------------------------------------------------------

% Departure 2: subscript n_ch, matching ATLAS-CONF-2022-023.
\newcommand*{\nch}{\ensuremath{n_{\text{ch}}}\xspace}
%\newcommand*{\nch}{\ensuremath{n^{\text{ch}}}\xspace}
\newcommand*{\Nch}{\ensuremath{N^{\text{ch}}}\xspace}
\newcommand{\mnch}{\mbox{$\langle n_{\text{ch}}\rangle$}\xspace}

\newcommand*{\ntrk}{\ensuremath{n_{\text{trk}}}\xspace}
\newcommand*{\nmix}{\ensuremath{n_{\text{trk}}^{\text{mix}}}\xspace}

\newcommand*{\pT}{\ensuremath{p_{\mathrm{T}}}\xspace}
\newcommand*{\ptch}{\ensuremath{p_{\mathrm{T}}}\xspace}%^{\mathrm{ch}}
\newcommand*{\sumpt}{\ensuremath{\sum\!p_{\mathrm{T}}^{\mathrm{ch}}}\xspace}
\newcommand*{\mT}{\ensuremath{m_{\mathrm{T}}}\xspace}

\newcommand*{\dphi}{\ensuremath{\Delta\varphi}\xspace}
\newcommand*{\dPhi}{\ensuremath{\Delta\phi}\xspace}
\newcommand*{\deta}{\ensuremath{\Delta\eta}\xspace}

\newcommand*{\pTOne}{\ensuremath{p_{\mathrm{T_{1}}}}\xspace}
\newcommand*{\pTTwo}{\ensuremath{p_{\mathrm{T_{2}}}}\xspace}

\newcommand*{\dd}{\ensuremath{\mathrm{d}}\xspace}

%-------------------------------------------------------------------------------
% Muon and dimuon variables
%-------------------------------------------------------------------------------

\newcommand*{\mmumu}{\ensuremath{m^{\mu\mu}}\xspace}
\newcommand*{\ptmumu}{\ensuremath{p_{\mathrm{T}}^{\mu\mu}}\xspace}
\newcommand*{\ymumu}{\ensuremath{y^{\mu\mu}}\xspace}
\newcommand*{\ptmu}{\ensuremath{p_{\mathrm{T}}^{\mu}}\xspace}
\newcommand*{\etamu}{\ensuremath{\eta^{\mu}}\xspace}
\newcommand*{\ptmuOne}{\ensuremath{p_{\mathrm{T}}^{\mu_{1}}}\xspace}
\newcommand*{\etamuOne}{\ensuremath{\eta^{\mu_{1}}}\xspace}
\newcommand*{\ptmuTwo}{\ensuremath{p_{\mathrm{T}}^{\mu_{2}}}\xspace}
\newcommand*{\etamuTwo}{\ensuremath{\eta^{\mu_{2}}}\xspace}
\newcommand*{\dzeromu}{\ensuremath{d_{0}^{\mu}}\xspace}
\newcommand*{\zzeromu}{\ensuremath{z_{0}^{\mu}}\xspace}
\newcommand*{\zvtxbar}{\ensuremath{\Bar{z}_{\mathrm{vtx}}}\xspace}
\newcommand*{\mubar}{\ensuremath{\Bar{\mu}}\xspace}

%-------------------------------------------------------------------------------
% Z-tagged observables (kept from the Z+UE analysis)
%-------------------------------------------------------------------------------

\newcommand*{\zz}{\ensuremath{\ell\ell}\xspace}
\newcommand*{\ptz}{\ensuremath{p_{\mathrm{T}}^{\ell\!\ell}}\xspace}
\newcommand*{\xz}{\ensuremath{x_{p}^{\ell\!\ell}}\xspace}
\newcommand*{\mz}{\ensuremath{m^{\ell\!\ell}}\xspace}
\newcommand*{\yz}{\ensuremath{y^{\ell\!\ell}}\xspace}
\newcommand*{\nz}{\ensuremath{n^{\ell\!\ell}}\xspace}
\newcommand*{\mptz}{\ensuremath{\langle p_{\mathrm{T}}^{\ell\!\ell} \rangle}\xspace}
\newcommand*{\zmu}{\ensuremath{Z\rightarrow \mu\mu}\xspace}
\newcommand*{\ze}{\ensuremath{Z\rightarrow ee}\xspace}
\newcommand*{\Dn}{\ensuremath{\Delta\bigl(\tfrac{1}{\nz}\tfrac{\dd\Nch}{\dd \Delta\varphi}\bigr)}\xspace}

%-------------------------------------------------------------------------------
% Draft mark-up
%-------------------------------------------------------------------------------

\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\green}{\color{green}}
\newcommand{\magenta}{\color{magenta}}
\newcommand{\orange}{\color{orange}}

%-------------------------------------------------------------------------------
% Standard ATLAS coordinate-system footnote.
% Not used by default in this proceedings; to include it, put
%   \note{\AtlasCoordFootnote}
% after \maketitle, or attach it with \footnote at the first use of eta.
%-------------------------------------------------------------------------------

\newcommand{\AtlasCoordFootnote}{%
ATLAS uses a right-handed coordinate system with its origin at the nominal
interaction point (IP) in the centre of the detector and the \(z\)-axis along
the beam pipe. The \(x\)-axis points from the IP to the centre of the LHC ring,
and the \(y\)-axis points upwards. Cylindrical coordinates \((r,\phi)\) are used
in the transverse plane, \(\phi\) being the azimuthal angle around the
\(z\)-axis. The transverse momentum is defined as
\(p_{\mathrm{T}} = \sqrt{p_x^2 + p_y^2}\), where \(p_x\) and \(p_y\) are the
momentum components along the \(x\)- and \(y\)-axes. The pseudorapidity is
defined in terms of the polar angle \(\theta\) as \(\eta = -\ln\tan(\theta/2)\),
and the rapidity as \(y = \tfrac{1}{2}\ln[(E+p_{z})/(E-p_{z})]\), where \(E\) is
the energy of a particle and \(p_{z}\) the momentum component along the beam
direction.}

